An Adaptive Multi-Layered Honeynet Architecture for Threat Behavior Analysis via Deep Learning

The escalating sophistication and variety of cyber threats have rendered static honeypots inadequate, necessitating adaptive, intelligence-driven deception. In this work, ADLAH is introduced: an Adaptive Deep Learning Anomaly Detection Honeynet designed to maximize high-fidelity threat intelligence while minimizing cost through autonomous orchestration of infrastructure. The principal contribution is offered as an end-to-end architectural blueprint and vision for an AI-driven deception platform. Feasibility is evidenced by a functional prototype of the central decision mechanism, in which a reinforcement learning (RL) agent determines, in real time, when sessions should be escalated from low-interaction sensor nodes to dynamically provisioned, high-interaction honeypots. Because sufficient live data were unavailable, field-scale validation is not claimed; instead, design trade-offs and limitations are detailed, and a rigorous roadmap toward empirical evaluation at scale is provided. Beyond selective escalation and anomaly detection, the architecture pursues automated extraction, clustering, and versioning of bot attack chains, a core capability motivated by the empirical observation that exposed services are dominated by automated traffic. Together, these elements delineate a practical path toward cost-efficient capture of high-value adversary behavior, systematic bot versioning, and the production of actionable threat intelligence.

==> tables/feature_analysis.tex <==
\begin{longtable}{l l l p{8cm}}
\toprule
\textbf{Feature} & \textbf{Data Type} & \textbf{Relevant} & \textbf{Justification} \\
\midrule
\endhead
\bottomrule
\endfoot
\_index & object & No & This is an internal metadata field for Elasticsearch and provides no information about the network traffic itself, making it irrelevant for threat analysis. \\
\_id & object & No & This is a unique document identifier in Elasticsearch and has no value for analyzing network threats. \\
\_score & object & No & This field represents the relevance score of a document in an Elasticsearch query and is not an intrinsic property of the network data. \\
\_ignored & object & No & This field lists fields that were not indexed because they were malformed. It is metadata about data ingestion, not the traffic itself. \\
sort & object & No & This field is used for sorting results in Elasticsearch and does not contain information about the network event. \\
src\_ip & object & Yes & Crucial for identifying the source of network traffic, which is a primary indicator for tracking attackers and recognizing distributed attacks. \\
dest\_ip\_geoip.geo.city\_name & object & Yes & Geographic information can help identify targeted attacks against specific locations and correlate threats with geopolitical factors. \\
dest\_ip\_geoip.geo.region\_name & object & Yes & Similar to city, region provides a broader geographical context, useful for identifying regional campaigns or filtering legitimate regional traffic. \\
dest\_ip\_geoip.geo.location.lat & float64 & Yes & Latitude provides precise geographic data, which can be used for mapping threats and can be a strong feature for clustering attacks spatially. \\
dest\_ip\_geoip.geo.location.lon & float64 & Yes & Longitude, along with latitude, gives a precise location of the destination IP, essential for spatial analysis of threats. \\
dest\_ip\_geoip.geo.continent\_code & object & Yes & A high-level geographic feature that can be useful for identifying continent-specific attack trends or policies. \\
dest\_ip\_geoip.geo.country\_iso\_code & object & Yes & Country code is a key feature for identifying nation-state actors or country-specific malware campaigns. \\
dest\_ip\_geoip.geo.postal\_code & object & No & Postal code is too granular and often unavailable or inaccurate for IP addresses, making it a noisy and unreliable feature. \\
dest\_ip\_geoip.geo.country\_name & object & Yes & Redundant if country_iso_code is used, but provides a human-readable country name. Its relevant, but one of the two should be chosen to avoid multicollinearity. \\
dest\_ip\_geoip.geo.timezone & object & Yes & Timezone can help infer the operational hours of attackers, which is a behavioral attribute that can be used for profiling. \\
TCP.res1 & float64 & No & This is a reserved field in the TCP header. It should be zero and has no defined meaning, making it irrelevant. \\
TCP.ack & object & Yes & The ACK flag is fundamental to the TCP handshake and state. Anomalous use of this flag can indicate scanning (e.g., ACK scan) or session hijacking attempts. \\
TCP.syn & object & Yes & The SYN flag is used to initiate connections. High rates of SYN packets from a source can indicate a SYN flood (DDoS) attack or network scanning. \\
TCP.psh & object & Yes & The PSH flag indicates that data should be pushed to the application immediately. It can be used in some forms of attacks or for data exfiltration. \\
TCP.urg & object & Yes & The URG flag indicates urgent data. While less common, it can be abused in attacks like the Urgent Pointer attack to bypass firewalls. \\
TCP.rst & object & Yes & The RST flag resets a connection. A large number of RST packets can indicate scanning activity (e.g., Xmas scan) or a rejection of connection attempts. \\
TCP.src\_port & float64 & Yes & Indicates the service or application generating the traffic on the source machine. High or ephemeral ports are normal for clients, but specific patterns can indicate malicious activity. \\
TCP.tcp\_flags & object & Yes & Provides a compact representation of all TCP flags. It is highly relevant, but potentially redundant if individual flag fields (SYN, ACK, etc.) are already used. \\
TCP.ack\_seq & float64 & Yes & The acknowledgment number is critical for understanding the state of a TCP session. Anomalies in sequence/acknowledgment numbers can reveal spoofing or session hijacking. \\
TCP.tcp\_options.tained & object & No & This seems to be a metadata flag from a specific security tool (e.g., Suricata) and may not generalize well. Its better to rely on more fundamental features. \\
TCP.tcp\_options.timestamp & object & Yes & TCP timestamps can be used to estimate system uptime and boot time, which can be used to fingerprint hosts. \\
TCP.tcp\_options.sack\_perm & object & Yes & Selective Acknowledgment Permitted. The presence or absence of this option can be used for OS fingerprinting. \\
TCP.tcp\_options.padding\_hex & object & No & Padding is used to align TCP options on a 32-bit boundary. Its content is generally not meaningful for threat analysis. \\
TCP.tcp\_options.nop & object & No & The No-Operation option is used for padding and has no intrinsic value for threat detection. \\
TCP.tcp\_options.window & object & Yes & The Window Scale option is part of the TCP handshake and can be used for passive OS fingerprinting (e.g., p0f). \\
TCP.tcp\_options.mss & object & Yes & Maximum Segment Size. The value of MSS is determined by the networking stack and can be a reliable indicator for OS and device fingerprinting. \\
TCP.window & float64 & Yes & The TCP window size is another parameter that varies between operating systems and can be used for passive fingerprinting. \\
TCP.cwr & object & Yes & Congestion Window Reduced flag. Part of the ECN mechanism, its usage can provide information about network congestion, which might be caused by certain attacks. \\
TCP.urg\_ptr & object & Yes & The urgent pointer, when the URG flag is set, can be used in attacks. A non-zero value is a significant event. \\
TCP.fin & object & Yes & The FIN flag is used to terminate connections. Unusual FIN flag usage can be a sign of a FIN scan. \\
TCP.dest\_port & float64 & Yes & The destination port indicates the target service. Port scanning and attacks against specific services (e.g., port 22 for SSH, 80 for HTTP) are identified by this feature. \\
TCP.hdr\_len & float64 & Yes & The TCP header length. A header length greater than the minimum (20 bytes) indicates the presence of TCP options, which can be used for fingerprinting. \\
TCP.ecn & object & Yes & Explicit Congestion Notification. Can be used for fingerprinting operating systems and might be used in some reconnaissance techniques. \\
TCP.checksum & object & No & The checksum is used for error detection. While an invalid checksum could indicate an issue, its typically handled by the network stack and is not a reliable feature for threat analysis, as it can be offloaded to hardware. \\
TCP.seq & float64 & Yes & The sequence number is fundamental to TCP. Predictable sequence numbers can be exploited in session hijacking attacks. Analyzing sequence numbers is key for deep packet inspection. \\
src\_port & float64 & Yes & This is a root-level copy of TCP.src_port or UDP.src_port. Its redundant if the protocol-specific field is used, but is generally a relevant feature. \\
FLOW.proxy\_ip & object & Yes & In a proxied environment, this indicates the internal proxy handling the connection, which can be useful context for localized threats. \\
FLOW.end & object & Yes & End timestamp of a flow, used with the start time to calculate duration. The timing of flows is a critical behavioral feature. \\
FLOW.start & object & Yes & Start timestamp of a flow. Crucial for calculating flow duration and analyzing the timing of events. \\
FLOW.bytes\_toclient & float64 & Yes & The volume of data sent from the server to the client. Unusually large values can indicate data exfiltration in reverse. \\
FLOW.backend\_ip & object & Yes & The actual server behind a proxy or load balancer. Knowing the true destination is important for internal threat analysis. \\
FLOW.proxy\_port & float64 & Yes & The port on the proxy service. Can help identify the specific proxy service involved in the connection. \\
FLOW.duration & float64 & Yes & The duration of a network flow. Very short flows can be indicative of scanning, while very long flows could be data transfers or persistent backdoors. \\
FLOW.bytes\_toserver & float64 & Yes & The volume of data sent from the client to the server. Large uploads can be a sign of data exfiltration or malware uploading. \\
FLOW.backend\_port & float64 & Yes & The port on the backend server. It clarifies the actual service being communicated with, which is essential context. \\
FLOW.reason & object & Yes & The reason a flow terminated (e.g., closed, timeout). A high number of timeouts could indicate a network problem or a stealthy scan. \\
FLOW.min\_rtt & float64 & Yes & Minimum Round-Trip Time. Provides an estimate of the latency to the other host, which can help in geolocation or identifying abnormal network paths. \\
FLOW.state & object & Yes & The state of the flow (e.g., new, established, closed). This is a fundamental feature for understanding the lifecycle of a connection. \\
src\_ip\_geoasn.as.number & float64 & Yes & The Autonomous System Number of the source IP. This helps to identify the network provider (e.g., a specific cloud provider, ISP), which is crucial context for attributing attacks. \\
src\_ip\_geoasn.as.organization.name & object & Yes & The name of the organization owning the ASN. It gives a human-readable context to the ASN, useful for identifying threats from known malicious networks. \\
log.offset & int64 & No & This is a metadata field indicating the position within a log file. It has no relevance to the network event itself. \\
log.file.path & object & No & The path of the source log file is metadata and not a feature of the network traffic. \\
dest\_port & float64 & Yes & This is a root-level copy of TCP.dest_port or UDP.dest_port. Redundant if protocol-specific fields are used, but highly relevant as it indicates the targeted service. \\
proto & object & Yes & The transport protocol (TCP, UDP, ICMP). This is one of the most fundamental features, as different protocols are used for different types of attacks. \\
dest\_ip & object & Yes & The destination IP address. Essential for identifying the target of an attack. \\
ecs.version & object & No & Elastic Common Schema version. This is metadata about the logging format, not the event. \\
observer.product & object & No & The product that observed the event. This is system metadata, not a feature of the traffic. \\
observer.version & object & No & The version of the observer. This is system metadata, not a feature of the traffic. \\
observer.type & object & No & The type of observer (e.g., sensor). This is system metadata, not a feature of the traffic. \\
observer.hostname & object & Yes & The hostname of the sensor that captured the data. This can be very important in a distributed environment to know which asset is being targeted. \\
xlog\_origin & object & No & A custom field indicating the origin of the log. This is metadata. \\
IP.version & float64 & Yes & IP protocol version (e.g., 4 or 6). Can be relevant as some threats are specific to IPv4 or IPv6. \\
IP.tot\_len & float64 & Yes & Total length of the IP packet. Packet size can be an indicator of certain activities, such as small packets for scanning or large packets for data exfiltration. \\
IP.tos & object & Yes & Type of Service field. Can be used for OS fingerprinting and to identify specific types of traffic that might be prioritized differently. \\
IP.dest\_addr & object & Yes & The destination IP address. This is redundant with the root-level dest_ip but is fundamentally a relevant feature. \\
IP.src\_addr & object & Yes & The source IP address. This is redundant with the root-level src_ip but is a crucial feature. \\
IP.id & object & Yes & IP Identification field. Can be used to reassemble fragmented packets and, in some cases, for OS fingerprinting (e.g., predictable IDs). \\
IP.hdr\_len & float64 & Yes & The IP header length. Similar to TCP header length, a value other than 20 bytes indicates IP options are present, which can be used for fingerprinting. \\
IP.ttl & float64 & Yes & Time-to-Live. The initial TTL value is characteristic of the source operating system, making it a very strong feature for OS fingerprinting. \\
IP.protocol & float64 & Yes & The protocol number (e.g., 6 for TCP, 17 for UDP). This is redundant with proto but is a fundamental networking feature. \\
IP.checksum & object & No & IP header checksum. Similar to the TCP checksum, its for error checking and not a reliable feature for threat analysis. \\
IP.flags & object & Yes & IP flags, especially the Dont Fragment (DF) and More Fragments (MF) bits. These are used in fragmentation-based attacks and for OS fingerprinting. \\
timestamp & object & Yes & The timestamp of the event. Essential for creating a timeline of an attack and for correlating events across different log sources. \\
timestamp\_processed & object & No & The time the event was processed by the logging pipeline. This is metadata and can introduce look-ahead bias if used as a feature. \\
backend\_id & object & No & An internal identifier for a backend system. Likely too specific to the logging infrastructure to be a generalizable feature. \\
SPLIT.split & object & No & Indicates if a log message was split. This is a logging infrastructure detail, not a network event feature. \\
event.original & object & No & The original, raw log message. This is a complex, unstructured field. While it contains all the information, the parsed fields are what should be used as features. Processing this directly is a separate, complex task (NLP). \\
src\_ip\_geoip.geo.country\_name & object & Yes & Geographic information for the source IP. As with the destination, this is important for identifying the origin of attacks and spotting geopolitical trends. \\
src\_ip\_geoip.geo.location.lat & float64 & Yes & Latitude of the source IP. Provides precise geographic origin for spatial analysis of attack sources. \\
src\_ip\_geoip.geo.location.lon & float64 & Yes & Longitude of the source IP. Provides precise geographic origin for spatial analysis of attack sources. \\
src\_ip\_geoip.geo.continent\_code & object & Yes & Continent of the source IP. Useful for high-level geographic filtering and analysis. \\
src\_ip\_geoip.geo.country\_iso\_code & object & Yes & Country code of the source IP. A critical feature for attributing attacks and recognizing country-specific campaigns. \\
src\_ip\_geoip.geo.timezone & object & Yes & Timezone of the source IP. Can help build a profile of an attackers likely working hours. \\
@version & object & No & Logstash metadata field. Not relevant for threat analysis. \\
origin & object & No & Origin system of the log (e.g., MADCAT). This is metadata. \\
host.containerized & bool & Yes & Indicates if the host is running in a container. This is important context, as container escapes are a specific type of threat. \\
host.mac & object & No & The MAC address of the host is a layer 2 detail and is generally not visible beyond the local network segment. It has limited value in analyzing IP-based threats from the internet. \\
host.name & object & Yes & Hostname of the reporting host. This is the same as observer.hostname and is critical for identifying the target asset. \\
host.architecture & object & Yes & The CPU architecture (e.g., x86_64, ARM). This is relevant because some malware is architecture-specific. \\
host.ip & object & Yes & The IP address(es) of the host that generated the log. Crucial for understanding which of my assets is involved in the event. \\
host.id & object & No & A unique ID for the host. This is metadata and is less useful than the hostname or IP address. \\
host.os.version & object & Yes & The full OS version. Highly relevant for vulnerability correlation, as many exploits are specific to certain OS versions and patch levels. \\
host.os.kernel & object & Yes & The kernel version. Very relevant for identifying vulnerability to kernel-level exploits. \\
host.os.family & object & Yes & OS family (e.g., debian, windows). High-level context that is very relevant for attack targeting. \\
host.os.name & object & Yes & The name of the operating system (e.g., Ubuntu). Relevant context for exploits. \\
host.os.codename & object & Yes & OS codename (e.g., jammy). Provides more specific version information. \\
host.os.platform & object & Yes & OS platform. Redundant with other OS fields but provides relevant context. \\
host.os.hostname & object & Yes & Redundant with host.name but provides the critical information of which asset is being observed. \\
input.type & object & No & Metadata from the logging agent (Filebeat) about the input source. Not a feature of the event. \\
ct\_status & object & Yes & Represents a Certificate Transparency status or a similar threat intelligence lookup. A status like Malicious would be a very strong feature. \\
unixtime & float64 & Yes & Unix timestamp of the event. Essential for temporal analysis, though may be redundant with @timestamp. \\
@timestamp & object & Yes & The primary timestamp for the event. Absolutely critical for any time-series analysis. \\
event\_type & object & Yes & A classification of the event (e.g., flow, syn_scan). This is a very high-value categorical feature, potentially a label from a pre-processing step. \\
agent.version & object & No & The version of the logging agent (e.g., Filebeat). This is operational metadata. \\
agent.name & object & No & The name of the logging agent. This is operational metadata. \\
agent.id & object & No & The ID of the logging agent. This is operational metadata. \\
agent.type & object & No & The type of the logging agent. This is operational metadata. \\
agent.hostname & object & No & The hostname where the agent is running. Redundant with host.name and observer.hostname, and is operational metadata. \\
agent.ephemeral\_id & object & No & An ephemeral ID for the agent instance. This is operational metadata. \\
tags & object & Yes & Tags can contain valuable, context-specific labels (e.g., _geoip_lookup_failure). These can be very strong features if they are consistent. \\
dest\_ip\_geoasn.as.number & float64 & Yes & The ASN of the destination IP. Important for understanding the network neighborhood of the target. \\
dest\_ip\_geoasn.as.organization.name & object & Yes & The organization owning the destination ASN. Provides context about the target (e.g., Deutsche Telekom AG, MICROSOFT-CORP-MSN-AS-BLOCK). \\
FLOW.payload\_hd & object & No & A hex dump of the flow payload. Like event.original, this is unstructured data that is difficult to use directly as a feature for most models without specialized processing. \\
FLOW.payload\_str & object & No & A string representation of the payload. While it contains potentially malicious content, its unstructured and better analyzed by signature-based systems or specialized models. Using it directly is problematic. \\
FLOW.payload\_sha1 & object & Yes & A SHA1 hash of the payload. This is a very strong feature. It can be used to identify known malicious payloads by checking against threat intelligence feeds. \\
host.os.type & object & Yes & The OS type (e.g., linux). Redundant with family/platform but relevant for identifying targeted attacks. \\
src\_ip\_geoip.mmdb.dma\_code & float64 & No & Designated Market Area code. This is a US-specific advertising metric and is too niche and noisy for general threat analysis. \\
src\_ip\_geoip.geo.city\_name & object & Yes & City of the source IP. Relevant for geographic analysis of attackers. \\
src\_ip\_geoip.geo.postal\_code & object & No & Postal code is too granular and often inaccurate for IP addresses, making it a noisy and unreliable feature. \\
src\_ip\_geoip.geo.region\_name & object & Yes & Region/state of the source IP. Good for geographic profiling. \\
TCP.payload\_hd & object & No & Hex dump of the TCP payload. Unstructured and difficult to use directly. The SHA1 hash is a better feature representation. \\
TCP.payload\_sha1 & object & Yes & SHA1 hash of the TCP payload. A very strong feature for identifying known malware or attack scripts. \\
TCP.payload\_str & object & No & String representation of the TCP payload. Unstructured data; better to use the hash or other derived features. \\
TCP.tcp\_options.eol & object & No & End of Option List. This is a protocol marker and carries no information. \\
icmp\_code & float64 & Yes & The ICMP code provides details about an ICMP message (e.g., host unreachable). It is crucial for interpreting ICMP-based scanning and reconnaissance. \\
ICMP.type\_str & object & Yes & A human-readable string for the ICMP type. Redundant with icmp_type but highly relevant. \\
ICMP.id & object & Yes & ICMP identifier, used to match echo requests with replies. Can be manipulated in some attacks. \\
ICMP.checksum & object & No & Checksum for error detection. Not a useful feature for threat analysis. \\
ICMP.code & float64 & Yes & Redundant with icmp_code, but fundamentally relevant. \\
ICMP.tainted & object & No & A metadata flag from a specific security tool. Better to use fundamental protocol features. \\
ICMP.type & float64 & Yes & The ICMP type number (e.g., 8 for echo request). Essential for understanding ICMP traffic (pings, traceroute, etc.). \\
ICMP.seq & object & Yes & ICMP sequence number, used to match echo requests and replies. Abnormal patterns can indicate malicious activity. \\
icmp\_type & float64 & Yes & Redundant with ICMP.type, but fundamentally relevant. \\
http.version & object & Yes & HTTP version. Can be used for fingerprinting clients and identifying protocol anomalies. \\
http.request.method & object & Yes & The HTTP method (GET, POST, etc.). Uncommon or malicious methods can indicate attacks like web shell interaction or vulnerability scanning. \\
user\_agent.original & object & Yes & The User-Agent string sent by an HTTP client. This is a very strong feature for identifying scanners (nmap, curl), malware, or specific client software. \\
user\_agent.os.full & object & Yes & Operating system parsed from the User-Agent string. Provides client context. \\
user\_agent.os.name & object & Yes & OS name parsed from User-Agent. Relevant client information. \\
user\_agent.name & object & Yes & Name of the agent (browser, tool) parsed from the User-Agent. Highly relevant. \\
user\_agent.device.name & object & Yes & Device type parsed from User-Agent. Can help distinguish between mobile, desktop, and bot traffic. \\
UDP.len & float64 & Yes & Length of the UDP datagram. Packet size can be relevant; for example, in amplification attacks. \\
UDP.src\_port & float64 & Yes & Source port for UDP traffic. Can indicate the client application or be part of a scan. \\
UDP.checksum & float64 & No & UDP checksum is optional and often zero. It is not a reliable feature. \\
UDP.dest\_port & float64 & Yes & Destination port for UDP traffic. Critical for identifying the targeted service (e.g., DNS on port 53). \\
url.original & object & Yes & The URL being accessed in an HTTP request. This is one of the most critical features for web attack detection, as it contains the path and query parameters where attacks (SQLi, XSS) are often embedded. \\
user\_agent.version & object & Yes & Version of the user agent. Can help identify outdated and vulnerable clients. \\
RAW.ether\_type & object & No & EtherType is a Layer 2 field. Its not typically relevant for IP-level threat analysis unless dealing with non-IP protocols. \\
RAW.pcap\_filter & object & No & The packet capture filter used. This is metadata about how the data was collected, not a feature of the event itself. \\
tainted & object & No & A generic tainted flag. Its unclear what this refers to and is likely tool-specific. Its better to use more explicit features. \\
SPLIT.part & float64 & No & Metadata about log splitting. Not a feature of the network event. \\
SPLIT.total & float64 & No & Metadata about log splitting. Not a feature of the network event. \\
SPLIT.tag & object & No & Metadata about log splitting. Not a feature of the network event. \\
ICMP.IP.version & float64 & Yes & Details of an IP packet encapsulated within an ICMP error message. This is highly relevant for diagnosing network issues and some attacks, as it shows the original packet that caused the error. \\
ICMP.IP.tos & object & Yes & TOS of the encapsulated packet. Relevant for fingerprinting the source of the original packet. \\
ICMP.IP.tot\_len & float64 & Yes & Total length of the encapsulated packet. \\
ICMP.IP.dest\_addr & object & Yes & Destination address of the encapsulated packet. Shows who the original packet was for. \\
ICMP.IP.src\_addr & object & Yes & Source address of the encapsulated packet. Shows who sent the original packet. \\
ICMP.IP.id & object & Yes & IP ID of the encapsulated packet. \\
ICMP.IP.hdr\_len & float64 & Yes & Header length of the encapsulated packet. \\
ICMP.IP.ttl & float64 & Yes & TTL of the encapsulated packet. \\
ICMP.IP.protocol & float64 & Yes & Protocol of the encapsulated packet. \\
ICMP.IP.flags & object & Yes & IP flags of the encapsulated packet. \\
ICMP.IP.checksum & object & No & Checksum of the encapsulated packet. Not a useful feature. \\
ICMP.TCP.res1 & float64 & No & Reserved field in an encapsulated TCP header. Irrelevant. \\
ICMP.TCP.ack & object & Yes & ACK flag of the encapsulated TCP packet. Provides context on the original session state. \\
ICMP.TCP.psh & object & Yes & PSH flag of the encapsulated TCP packet. \\
ICMP.TCP.syn & object & Yes & SYN flag of the encapsulated TCP packet. \\
ICMP.TCP.urg & object & Yes & URG flag of the encapsulated TCP packet. \\
ICMP.TCP.src\_port & float64 & Yes & Source port of the encapsulated TCP packet. \\
ICMP.TCP.tcp\_flags & object & Yes & TCP flags of the encapsulated packet. \\
ICMP.TCP.rst & object & Yes & RST flag of the encapsulated TCP packet. \\
ICMP.TCP.ack\_seq & float64 & Yes & Ack number of the encapsulated TCP packet. \\
ICMP.TCP.window & float64 & Yes & Window size of the encapsulated TCP packet. \\
ICMP.TCP.cwr & object & Yes & CWR flag of the encapsulated TCP packet. \\
ICMP.TCP.urg\_ptr & object & Yes & Urgent pointer of the encapsulated TCP packet. \\
ICMP.TCP.fin & object & Yes & FIN flag of the encapsulated TCP packet. \\
ICMP.TCP.dest\_port & float64 & Yes & Destination port of the encapsulated TCP packet. Vital for understanding the original target. \\
ICMP.TCP.hdr\_len & float64 & Yes & Header length of the encapsulated TCP packet. \\
ICMP.TCP.ecn & object & Yes & ECN flag of the encapsulated TCP packet. \\
ICMP.TCP.checksum & object & No & Checksum of the encapsulated TCP packet. Not useful. \\
ICMP.TCP.seq & float64 & Yes & Sequence number of the encapsulated TCP packet. \\
ICMP.unused & object & No & An unused field in the ICMP header. Irrelevant. \\
ICMP.code\_str & object & Yes & The human-readable ICMP code string. Highly relevant for context. \\
ICMP.TCP.tcp\_options.tained & object & No & Tool-specific metadata on an encapsulated packet. Irrelevant. \\
ICMP.TCP.tcp\_options.mss & object & Yes & MSS from an encapsulated TCP packet. Relevant for fingerprinting. \\
ICMP.TCP.tcp\_options.padding\_hex & object & No & Padding from an encapsulated TCP packet. Irrelevant. \\
http.request.referrer & object & Yes & The HTTP referrer can reveal the previous site the user came from, which is useful for tracking attack paths or identifying malicious redirection. \\
ICMP.TCP.tcp\_options.nop & object & No & NOP from an encapsulated TCP packet. Irrelevant. \\
ICMP.TCP.tcp\_options.timestamp & object & Yes & Timestamp from an encapsulated TCP packet. Relevant for fingerprinting. \\
\end{longtable}
